Simulation of Dynamic Environments for SLAM

Simulation engines are widely adopted in robotics. However, they lack either full simulation control, ROS integration, realistic physics, or photorealism. Recently, synthetic data generation and realistic rendering has advanced tasks like target tracking and human pose estimation. However, when focusing on vision applications, there is usually a lack of information like sensor measurements or time continuity. On the other hand, simulations for most robotics tasks are performed in (semi)static environments, with specific sensors and low visual fidelity. To solve this, we introduced in our previous work a fully customizable framework for generating realistic animated dynamic environments (GRADE) [1]. We use GRADE to generate an indoor dynamic environment dataset and then compare multiple SLAM algorithms on different sequences. By doing that, we show how current research over-relies on known benchmarks, failing to generalize. Our tests with refined YOLO and Mask R-CNN models provide further evidence that additional research in dynamic SLAM is necessary. The code, results, and generated data are provided as open-source at https://eliabntt.github.io/grade-rrSimulation of Dynamic Environments for SLAM

==> approach.tex <==
\section{Approach}
\label{sec:approach}

To simulate a dynamic world we need: a set of assets, a coherent placement of the moving objects, a robot that we can control, a fully controllable simulation, and, finally, being able to save and process the generated data. However, no current simulation framework or software allows such an approach seamlessly. In this work, we show how we address all these aspects by providing APIs and tools to customize and expand each step of the pipeline. This will allow researchers to integrate and adapt GRADE to their workflows, using custom robots and environments, place and control dynamic assets, and add sensors and noise models while being in customizable, physically-enabled and realistically-rendered dynamic worlds with full control of the simulation itself and instantaneous access to ground truth data. With our framework they will also be able to repeat each experiment while changing its conditions and recording additional information.

The environment or any other asset can be created beforehand in a variety of applications. In this regard, we provide ways to directly import objects and animated humans (\secref{subsec:dynamicassets}) from different datasets, use environments developed for UE (Sec.~\ref{subsec:savana}), obtained from online sources (\secref{subsec:scenarios}), or loaded through Blender (\secref{sec:envdatagen}). Leveraging the Omniverse Connectors\footnote{\url{https://bit.ly/3X82sph}} and the adoption of the Universal Scene Description (USD) format, we convert and load all of them in Isaac Sim. Through the simulation software, we are able to change lighting (including foggy conditions or auto-exposure) and rendering settings, light colors and intensity, materials' reflections parameters, assets' textures, and the time of day. A schematic of the tools we developed is depicted in Fig.~\ref{fig:pipeline} and more detailed in Fig.~\ref{fig:pipeline2}.

\begin{figure}[!th]
    \centering
    \includegraphics[width=0.5\textwidth]{fig/pipeline1.png}
    \caption{A visual description of GRADE and how it integrates with the USD format. The modules we developed are in color.}
    \label{fig:pipeline}
\end{figure}

\begin{figure*}[!th]
    \centering
    \includegraphics[width=\textwidth]{fig/pipeline2.png}
    \caption{A detailed scheme of GRADE's workflow which shows how each tool can be adapted to everyone's need.}
    \label{fig:pipeline2}
\end{figure*}

Given an environment and an animated asset, it is necessary to avoid any physical overlap between the two. To do so, we employ the full 3D trace of the animation sequence and check for any co-penetration between the meshes. This was more effective than using the 2D occupancy projection since we employ clothing animations and diversified actions that would greatly increase the occupancy footprint itself while not necessarily colliding with objects. Alternatively, the animation can be placed manually in the environment, as we do in Sec.~\ref{subsec:savana}, predefined locations defined through the code can be used, or other strategies can be easily implemented within our work. 

The robot can be created directly in Isaac Sim by adding joints to any object, or by using the common URDF file format. We show how to control it through teleporting, by velocity and position setpoints using Isaac Sim's internal PD control, by using one of the pre-build models, or through rigid non-physics transformations (as a flying object). Software in the loop also works, e.g. by using \textit{MoveIt}~\cite{moveit} for robotic arms. However, we note that Isaac Sim does not provide fluid-dynamic physics and, like Gazebo, it does not model frictionless perpendicular translation movements~\cite{irotate}, necessary for omnidirectional wheels. However, ROS is fully embedded in the simulation engine and this allowed us to use custom software in the loop by exploiting the communication system and the joint definitions. Indeed, we developed a generalized control framework that, given a position or a velocity setpoint as input, can output 6 degrees of freedom (DOF) joint velocity commands using a PID formulation. We then equip our robots in Isaac Sim with 6 joints, controlled by the simulation engine itself, that are physically enabled, with custom stiffness, damping and force settings, and that can move the robot freely. In this way, we can receive setpoints from other control software, e.g. (N)MPC formulations, and translate that to joint, and thus robot, movements. The sensors of the robot can then be defined either beforehand or loaded and modified dynamically at simulation time. Thanks to this, we already implemented a seamless way to import multiple robots and allow their independent control. This is obtained by contextually changing the used ROS topics employed by each robot at runtime using unique names. An example of this implementation is our multi-robot scenario described in~\ref{subsec:scenarios}. We also want to stress the fact that the control can be \textit{with} or \textit{without} physics, as well as \textit{with} or \textit{without} ROS, increasing the flexibility of our framework.

We then set up and control all aspects of the simulation through a single Python script. This includes starting the simulation, loading any asset, personalizing every setting and applying any desired customization, stepping the simulation (physics and rendering step), launching ROS nodes, and full supervision on when and which information we want to publish and save. We can easily record the data through \textit{rosbags} or save it directly to the hard drive from the simulation itself, as well as including any other custom software or package. 

Post-processing is then necessary to effectively test any method. To this end, we made a set of tools available to add noise and process the data. Specifically:
i) IMU noise and bias, ii) color camera motion blur, and rolling shutter noise, iii) depth filtering and noise based on customizable settings. This can be easily expanded to different sensors (e.g. LRF, odometer), used to modify the saved data after the experiment is completed, or integrated directly into the simulation to publish noisy data alongside the corresponding ground truth.

We then provide a way to precisely replay any experiment. This includes moving the robot, the objects, and the humans at the exact recorded location for every simulation step while keeping a physically enabled environment. This allows the generation of new ground truth data from any simulated run from previously existing sensors, such as normals or optical flow, or from new sensors, like a newly added camera or a LiDAR. One can also modify the experiment itself, for example by employing different light colors or visual settings, or by adding a new robot. 

Finally, we provide code to export all SMPL parameters and any skeleton information from the selected experiment, easily visualize the recorded data, map semantic and instance information to different classes, and prepare data to train neural networks.

==> generation.tex <==
\section{Data Generation}
\label{sec:gen}

Using the system introduced in GRADE~\cite{GRADE}, we generated an indoor dynamic environment dataset that we proceed to describe. We structured our work in such a way that every step is interchangeable with custom implementations and different strategies, including working completely without ROS, physics, or other software in the loop. An example of the data generated can be seen in Fig.~\ref{fig:gendata}.

\subsubsection{Environments}
\label{sec:envdatagen}
As shown in Sec.~\ref{soa:envs}, there are only a few publicly available environment datasets that have realistic lighting and textured meshes. The only \textit{free} viable solution we found is the 3D-Front~\cite{3d-front} dataset. We loaded the scenes into Blender using an enhanced \textit{blenderproc} loader. The environments are randomized with \textit{ambientCG}\footnote{\url{https://ambientcg.com/}} textures. Once the scene is loaded, we compute the circumscribed rectangle and the approximated enclosing non-convex polygon. To that end, we first assume convex boundaries, find an enclosing convex polygon and transform it to non-convex if the angle between two subsequent vertices is different from 90 degrees. This is just an approximation which does not capture all situations, such as small alcoves, but for our use-case this is enough. We then export the STL and x3d files of the environment. The x3d format can then be easily converted to an octomap~\cite{octomap}. The STL file, the polygon vertices and the inscribing rectangle are then used during the assets' placement procedure. For other environments, e.g. from Unreal Engine (or any other modelling software), downloaded from online sources, or digital twins, a similar procedure can be applied, as exemplified in~\secref{subsec:scenarios}.

\subsubsection{Dynamic assets}\hfill
\label{subsec:dynamicassets}

\textbf{Humans:}
In our work, we decided to employ human animations from two main datasets. The first one, Cloth3D, comprises various animated sequences with clothed SMPL models. The second one is AMASS's SMPL \textit{unclothed} fittings over the CMU dataset. We randomize the appearance of the assets by using Surreal's SMPL textures, which are, although low-resolution, also freely available. We then load the animation sequence in Blender and export it as a USD file with a tool that we developed. Cloth3D animations are exported as deformed vertex mesh sequences, while AMASS fittings as sequences of skeleton joint transformations. We then generate a 3D trace of the animation and export it as an STL file. All information like SMPL parameters, vertices locations, and length of the sequence is exported contextually or can be re-generated at any time. 

\textbf{Objects:} We use two sources of additional objects in our simulation, namely Google Scanned Objects and ShapeNet. This increases variability in the simulation and more difficult scenarios. Those objects are treated as random flying objects. For simplicity, we do \textit{not} restrict those objects to not collide with other parts of the environment.


\subsubsection{Placement of dynamic assets}
The procedure we created to place the humans is based on the exported STLs of the environment and of each animation sequence. We use MoveIt's~\cite{moveit} interface of the Flexible Collision Library (FCL) to check if there is a collision between any given couple of STL meshes. That is, given a set of animated humans that need to be placed in the scene, the animation sequences are randomly positioned one after the other while checking for collision between them, the environment or with any already placed one. We consider a threshold value below which a collision is not considered, avoiding rejecting intersections with small objects like plant leaves, and set this threshold to 200 contact points. Using STLs allows us to correctly account for the 3D occupancy of clothes and wide movements of arms and legs instead of relying on their simple projected 2D occupancy. By design, flying objects are loaded and randomly rigidly animated, without considering any possible collision. Both the placement of the humans and the control of the flying object can be customized, including enabling collisions for the latest.

\subsubsection{Robot description and control}
\label{subsec:robotdescrcontrol}
Any robot could be loaded into the simulation. To simulate a freely moving camera that automatically explores the environments we use a drone model, controlled by six independent joints, using an active SLAM framework. To this end, we employ the Firefly drone from RotorS~\cite{rotors} and control it with our custom 6DOF controller described in Sec.~\ref{sec:approach}. We use the FUEL~\cite{zhou2021fuel} framework to autonomously explore the environment. FUEL's exploration goals are supplied to a NMPC~\cite{kamelmpc2016} to predict a realistic trajectory for the robot. The final predicted state is then provided to our controller, which supplies commands to the joints limited in speed and range as in Tab.~\ref{tab:limits}. The initial location of the robot is randomized, and its initial orientation is pre-optimized to avoid pointing towards empty space, i.e. directly towards a window. Due to flying objects and the unpredictability of moving subjects, sometimes the drone goes `through' dynamic assets. Although a way to avoid this would be to pre-sample valid trajectories, we see this as an opportunity to develop more reliable systems. Indeed, these events cause situations, such as losing track of the features due to completely black images or sudden changes between frames, which usually remain untested since not present in currently available datasets. However, those are possible scenarios that can occur if one considers real hardware or communication links that might fail or degrade or real-world environments in which animals or anything else could cause occlusions of the camera lens even for a brief moment. Nonetheless, we are not aware of any data currently available that pose such a challenge. Note that, by offering the possibility of repeating experiments, one can solve this issue by simply re-generating the occluded frames.

\begin{table}[!h]
\centering
\begin{tabular}{l|c|c|c}
 & x, y, z & roll, pitch & yaw \\
\hline
Position & Env. limits & $[-25,25]$ or $[0,0]$ degrees & $[0,360]$ degrees \\
Speed & $0.5$ m/s & $40$ deg/s & $30$ deg/s
\end{tabular}
\caption{Joint limits}
\label{tab:limits}
\end{table}

\subsubsection{Simulation management}
We manage the simulation through a single python script with various submodules. The script communicates via ROS with the other software packages to complete the system. %Thanks to its modularity, every module or option can be disabled or exchanged with custom implementations. 
First, we load the environment, center it w.r.t. the origin, and generate the 2D occupancy map. In this, we also define the size of the physics step, i.e. how much the clock will advance during every loop of the simulation, and rendering parameters, e.g. auto-exposure or path/ray-tracing settings. In our simulations the physics step corresponds to 1/240-th of a second. Second, we randomize lights' colors, intensities, and surface roughness (i.e. reflection capabilities). Third, we load the robot, move it to the starting location, which can be either random or pre-defined, and attach its specific set of sensors (including the cameras), ROS publishers, and motion controller. The robot is controlled according to the description provided in Sec.~\ref{subsec:robotdescrcontrol} with either full 6 DOF capabilities or with a stabilized flight (without roll and pitch). Then, we import a random number of people and randomly place the animations within the environment. If a person cannot be placed due to detected collisions, it is then removed from the simulation. If desired, we can load and animate rigid objects. The number of flying objects loaded varies based on the experiment settings. Overall, accounting for the degrees of freedom of the robot and the presence of flying objects, we obtain six different scenarios. In this work, each experiment sequence can indeed be identified by the usage of N (no) F (few) L (lot) letters, indicating the number of obstacles, and the presence of the letter H, which indicates a stabilized flight of the drone. This is summarized in Tab.~\ref{tab:combinations}. We then enter the main simulation loop. In that, we set a $1$ second (of simulation time) bootstrap period for every experiment to randomize the initial conditions of the robot. When the bootstrap sequence ends, we publish a single message to signal the start of the experiment and record data for one minute. In the main simulation loop we advance the physics one step at a time, manually control the animation timeline, publish the ROS information at the desired rates (based on the physics step) and write data to the disk. A full description of the data that we save with the corresponding FPS is in Tab.~\ref{tab:pubfreq}. The scene is rendered with path tracing and auto exposure. The rendering speed greatly depends on the number of lights, reflections, assets in the scene, and cameras. We use two cameras with the same horizontal and vertical FOV, one low resolution ($640 \times 480$) and one high resolution ($1920 \times 1080$). Across different architectures, rendering each \textbf{couple} of views took an average of 12 seconds, including the time necessary to get the remaining ground truth information such as the instance information. However, by tuning the simulation parameters, one can improve that to multiple images per second  up to processing times which are faster than 15 FPS. In this, the physics simulation step causes a noticeable delay~\cite{nvidiaSlowSpeeding} whenever high-frequency messages related to physics need to be published (e.g. the IMU) due to its tiding with the USD files and the necessity to constantly read and write information to them~\cite{nvidiaSlowSpeeding}. The low-resolution RGB and depth are published with ROS and saved with the \textit{rosbag} tool. The high-resolution camera is used to save groundtruth data with \textit{numpy} arrays such as 2D and 3D bounding boxes, instance segmentation masks, camera pose, as well as RGB and depth. All of these can also be published as ROS topics. The animations are reversed based on the average movement duration to increase variability and avoid too many static figures.

\begin{table}[]
\centering
\setlength\tabcolsep{3pt}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c|c|c|c}
\textbf{Sensor} & 
Clock &
\begin{tabular}[c]{@{}c@{}}IMU\\ body/camera\end{tabular} & 
TF  & 
\begin{tabular}[c]{@{}c@{}}Joint\\ state\end{tabular} &
\begin{tabular}[c]{@{}c@{}}Camera\\ pose\end{tabular} & 
Odometry & 
RGB &
Depth &
\begin{tabular}[c]{@{}c@{}}Starting\\ Experiment\end{tabular}   \\ \hline
\textbf{FPS} &
240 &
240 & 
120 &
120 &
60 &
60 &
30 & 
30 &
once 
\end{tabular}}
\caption{Publish frequency for each one of the sensor recorded}
\label{tab:pubfreq}
\end{table}


\begin{table}[!h]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c}
& 
Humans & 
GSO & 
ShapeNet &
Horizontal & 
Free & Sequences \\
\hline
N & 7-40 & 0 & 0 & & \tick & 63 \\
\hline
HN & 7-40 & 0 & 0 & \tick & & 77 \\
\hline
F &  7-40 & 5 & 5 & & \tick & 44 \\
\hline
HF & 7-40 & 5 & 5 & \tick & & 63 \\
\hline
 L & 7-40 & 10 & 10 & & \tick & 34 \\
\hline
HL & 7-40 & 10 & 10 & \tick & & 63 \\
\end{tabular}}
\caption{Generation summary. N/F/L: No/Few/Lot obstacles, H: horizontal. The number of humans loaded \textit{before} placement is random between 7 and 40. GSO: Google Scanned Objects.}
\label{tab:combinations}
\end{table}

\begin{figure*}[!ht]
  \includegraphics[width=0.245\textwidth, height=2.8cm]{fig/rgb_conv.jpg}
  \includegraphics[width=0.245\textwidth, height=2.8cm]{fig/depth_conv.jpg}
  \includegraphics[width=0.245\textwidth, height=2.8cm]{fig/motion.jpg}
  \includegraphics[width=0.245\textwidth, height=2.8cm]{fig/normal.jpg}
  
  \vspace{3pt}
  
  \includegraphics[width=0.245\textwidth, height=2.8cm]{fig/bbox2d_conv.jpg}
  \includegraphics[width=0.245\textwidth, height=2.8cm]{fig/instance_conv.jpg}
  \includegraphics[width=0.245\textwidth, height=2.8cm]{fig/sem_conv.jpg}
  \includegraphics[width=0.245\textwidth, height=2.8cm]{fig/SMPL.png}
  \caption{An example of the generated data following the pipeline described in Sec.~\ref{sec:gen}, using one of the 3D-Front environments. In the top row, from the left, we can see the rendered RGB image, corresponding depth map, optical flow, and surface normals. In the bottom row, starting from the left, we show 2D bounding boxes, semantic instances, semantic segmentation, and SMPL shapes. Best viewed in color.}
  \label{fig:gendata}
\end{figure*}


\begin{figure*}[!ht]
  \includegraphics[width=0.195\textwidth, height=3cm]{fig/rgb-sav.png}
  \includegraphics[width=0.195\textwidth, height=3cm]{fig/rgb-road.png}
  \includegraphics[width=0.195\textwidth, height=3cm]{fig/rgb-r1.png}
  \includegraphics[width=0.195\textwidth, height=3cm]{fig/rgb-r2.png}
  \includegraphics[width=0.195\textwidth, height=3cm]{fig/rgb-r3.png}
  
    \vspace{3pt}
    
  \subcaptionbox{Zebras in a savanna\label{img:scen_zebra}}{\includegraphics[width=0.195\textwidth, height=3cm]{fig/inst-sav.png}}\hfill
  \subcaptionbox{People in a city\label{img:scen_city}}{\includegraphics[width=0.195\textwidth, height=3cm]{fig/inst-road.png}}\hfill
  \subcaptionbox{Multi-robot: ground robot\label{img:scen_gr1}}{\includegraphics[width=0.195\textwidth, height=3cm]{fig/inst-r1.png}}\hfill
  \subcaptionbox{Multi-robot: drone \#1\label{img:scen_gr2}}{\includegraphics[width=0.195\textwidth, height=3cm]{fig/inst-r2.png}}\hfill
  \subcaptionbox{Multi-robot: drone \#2\label{img:scen_gr3}}{\includegraphics[width=0.195\textwidth, height=3cm]{fig/inst-r3.png}}
  
  \vspace{8pt}
  
  \caption{The scenarios we tested: zebras in a savanna, people in a city environment, and a multi-robot scenario (ground, 1st drone, 2nd drone). The RGB are in the top row and the corresponding instance segmentations (randomly colored) are in the bottom one. For the last two images, we highlight the other robots in the field of view with a red box. Better viewed in color.}
  \label{img:scenarios}
\end{figure*}

\subsubsection{Post-processing}
Post-processing includes three steps: i) selecting the correct \textit{rosbag} portion, ii) re-indexing the bags, and iii) adding noise to IMU (inspired by~\cite{deblurDatasetIMU}), depth and RGB data. Re-indexing is necessary due to an issue that comes from the Isaac simulator itself. The clock message is not always published promptly, causing the wrong timing of some subsequently published ROS messages. This happens especially for messages which are published at the same rate as the clock time, which, in our case, are the IMU ones. However, re-indexing is possible by using the message index number and using these to obtain correct the time stamps. Briefly pausing the script each time the clock is published can easily solve this issue. 


\subsection{Evaluated scenarios}
\label{subsec:scenarios}
We evaluated four additional scenarios to demonstrate how GRADE can be used in various ways by combining different techniques. We based those on what we described above by modifying the main simulation loop, including additional options, e.g. for control or asset placements, and testing different environments. This highlights the flexibility of the GRADE framework and how it can be used effectively to simulate a variety of scenarios and thus be used to address several research topics.

\subsubsection{Outdoor - Savanna}
\label{subsec:savana}
We test our pipeline by generating data in a savanna environment\footnote{\url{https://bit.ly/3i5j6Hi}} with several simulated animated zebras. The environment was obtained from Unreal Engine and converted manually to the USD format. The zebra asset and a set of base animations were available on Sketchfab\footnote{\url{https://bit.ly/3Ijpzc3}}. Using Blender, we exported four animations, namely walking, eating, trotting and jumping, to the USD format. Then, three different transitions between i) walking, ii) eating, iii) trotting, iv) jumping, and v) idle states have been manually created in Isaac Sim using the animation timeline tool. We then placed the assets manually in the main environment USD file (Fig.~\ref{img:scen_zebra}). In that way, we can avoid the placement step since the animations are loaded in the simulation directly with the world file. We then extended our code base to load the robot at a specified initial location and scripted a sequence of waypoints for each one of the robot's joints. Those waypoints are then provided to the Isaac engine directly from the main simulation loop as position/orientation goals, without any external intervention or software in the loop, while still being affected by the physics of the simulation. Thus, here we avoided any integration with external ROS packages or usage of any other control software.

\subsubsection{Outdoor - City}
\label{subsec:city}
By using the same placement strategy used for the original dataset, we position 99 humans and use FUEL to record an `exploration' sequence in an outdoor city-like environment\footnote{\url{https://bit.ly/3WKYBOS}} (Fig.~\ref{img:scen_city}). With this experiment, we aim to show the scalability of the system. 

\subsubsection{Ground robot Active SLAM}
\label{subsec:irotate}
To prove the adaptability of GRADE to different platforms and SIL, we decided to use our framework with the \textit{iRotate} package~\cite{irotate} for active SLAM exploration of an indoor environment. The world was obtained from Sketchfab\footnote{\url{https://bit.ly/3VKJ6FF}}, converted using our tool developed for Blender and was kept static. Robotino robot's URDF was imported in Isaac Sim and controlled with the original four joints (x, y, robot\_yaw, camera\_yaw) by using the same 6DOF custom controller (see Sec.~\ref{sec:approach}, Sec.~\ref{subsec:robotdescrcontrol}), but this time with velocity setpoints. Using our custom controller was necessary since Isaac lacked omnidirectional wheels with the capability of having frictionless perpendicular movement, necessary in three-wheeled omnidirectional robot. As in Gazebo, we can independently control the robot and the camera yaw movements and explore the environment with our previously developed software. This by just adapting the topics used by \textit{iRotate}~\cite{irotate} with minimal modifications of the main simulation loop to account for additional sensors, e.g. the laser range finder.

\subsubsection{Multi-robot}
\label{subsec:multirobot}
To show how we can simulate multi-robot scenarios in GRADE, we loaded two drones (Fig.~\ref{img:scen_gr3} and Fig.~\ref{img:scen_gr2}) and a ground omnidirectional robot (Fig.~\ref{img:scen_gr1}) in the same indoor environment. By introducing a parameter to identify the type of robot, in a single loop we import and place those in the environment, equip them with their specific sensor suite, attach to each one unique ROS topics and launch the corresponding control software. Each flying robot was indeed controlled by FUEL as in the main data generation loop, while the ground robot was controlled using \textit{iRotate}.

\begin{table*}[ht]
    \centering
    \resizebox{\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc|cc|cc|cc|cc}
  & \multicolumn{2}{c|}{\begin{tabular}{@{}c@{}}Dynamic \\ VINS (VIO) \end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}{@{}c@{}}Dynamic \\ VINS (VO) \end{tabular}} & \multicolumn{2}{c|}{TartanVO} & \multicolumn{2}{c|}{StaticFusion} & \multicolumn{2}{c|}{DynaSLAM} & \multicolumn{2}{c|}{ORB-SLAMv2}& \multicolumn{2}{c}{RTABMap} \\
Sequence & ATE [m] & \begin{tabular}{@{}c@{}}Missing \\ Time [s]\end{tabular} & ATE [m] & \begin{tabular}{@{}c@{}}Missing \\ Time [s]\end{tabular} & ATE [m] & \begin{tabular}{@{}c@{}}Missing \\ Time [s]\end{tabular} & ATE [m] & \begin{tabular}{@{}c@{}}Missing \\ Time [s]\end{tabular} & ATE [m] & \begin{tabular}{@{}c@{}}Missing \\ Time [s]\end{tabular} & ATE [m] & \begin{tabular}{@{}c@{}}Missing \\ Time [s]\end{tabular} & ATE [m] & \begin{tabular}{@{}c@{}}Missing \\ Time [s]\end{tabular} \\ \hline
FH  & 0.155 & 1.03 & 0.367 & 0.43 & 0.582 & 0.00 & 0.854 & 0.00 & 0.309 & 1.50 & 0.386 & 0.00 & 0.097 & 1.97\\
F  & 0.886 & 1.27 & 1.857 & 1.37 & 4.223 & 0.00 & 3.992 & 0.00 & 0.178 & 49.67 & 0.144 & 44.30 & 0.125 & 47.03\\ 
DH  & 1.681 & 0.43 & 1.183 & 3.30 & 1.234 & 0.00 & 1.091 & 0.00 & 0.002 & 57.33 & 0.005 & 56.80 & 0.013 & 49.13\\ 
D  & 0.707 & 0.67 & 1.598 & 1.63 & 1.356 & 0.00 & 2.278 & 0.00 & 0.043 & 26.93 & 0.700 & 11.07 & 0.405 & 28.77\\
WOH & 0.491 & 1.03 & 0.871 & 1.23 & 2.399 & 0.00 & 1.826 & 0.00 & 0.023 & 28.53 & 0.022 & 27.90 & 0.101 & 27.93 \\
WO  & 1.086 & 2.63 & 1.163 & 3.17 & 2.473 & 0.00 & 2.213 & 0.00 & 0.119 & 55.23 & 0.171 & 48.23 & 0.075 & 50.70\\
SH  & 0.419 & 0.57 & 0.069 & 0.43  & 2.517 & 0.00 & 4.184 & 0.00 & 0.016 & 0.00 & 0.018 & 0.00 & 0.072 & 0.00\\ 
S  & 0.177 & 0.57 & 0.137 & 0.43  & 1.308 & 0.00 & 3.538 & 0.00 & 0.029 & 0.00 & 0.026 & 0.00 & 0.133 & 0.00\\
\end{tabular}}
    \caption{ATE RMSE [m] and missing time [s] of the tested \textbf{noisy} sequences. Each experiment is 60 seconds long. \bigskip}
    \label{tab:slamnoisy}
\end{table*}

\begin{table*}[ht]
    \centering
    \resizebox{\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc|cc|cc|cc|cc}
  & \multicolumn{2}{c|}{\begin{tabular}{@{}c@{}}Dynamic \\ VINS (VIO) \end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}{@{}c@{}}Dynamic \\ VINS (VO) \end{tabular}} & \multicolumn{2}{c|}{TartanVO} & \multicolumn{2}{c|}{StaticFusion} & \multicolumn{2}{c|}{DynaSLAM} & \multicolumn{2}{c|}{ORB-SLAMv2}& \multicolumn{2}{c}{RTABMap} \\
Sequence & ATE [m] & \begin{tabular}{@{}c@{}}Missing \\ Time [s]\end{tabular} & ATE [m] & \begin{tabular}{@{}c@{}}Missing \\ Time [s]\end{tabular} & ATE [m] & \begin{tabular}{@{}c@{}}Missing \\ Time [s]\end{tabular} & ATE [m] & \begin{tabular}{@{}c@{}}Missing \\ Time [s]\end{tabular} & ATE [m] & \begin{tabular}{@{}c@{}}Missing \\ Time [s]\end{tabular} & ATE [m] & \begin{tabular}{@{}c@{}}Missing \\ Time [s]\end{tabular} & ATE [m] & \begin{tabular}{@{}c@{}}Missing \\ Time [s]\end{tabular} \\ \hline
FH  & 0.069 & 0.67 & 0.201 & 0.43 & 0.551 & 0.00 & 0.085 & 0.00 & 0.241 & 3.43 & 0.149 & 0.00 & 0.126 &  0.00 \\ 
F   & 0.647 & 1.20 & 1.337 & 2.93 & 4.132 & 0.00 & 2.866 & 0.00 & 0.147 & 49.23 & 0.431 & 39.10 & 0.115 &  46.93\\ 
DH  & 8.103 & 0.43 & 1.178 & 8.17 & 1.259 & 0.00 & 1.664 & 0.00 & 0.008 & 57.07 & 0.005 & 48.53 & 0.094 &  21.63 \\ 
D   & 0.188 & 0.67 & 1.304 & 0.83 & 1.264 & 0.00 & 1.212 & 0.00 & 0.057 & 6.33 & 0.459 & 0.30 & 0.492 &  7.07 \\
WOH & 0.239 & 1.10 & 1.272 & 1.00 & 2.361 & 0.00 & 1.980 & 0.00 & 0.015 & 27.70 & 0.012 & 27.73 & 0.042 &  25.87 \\
WO  & 0.501 & 2.20 & 0.985 & 3.47 & 2.380 & 0.00 & 2.807 & 0.00 & 0.083 & 55.20 & 0.163 & 48.23 & 0.053 &  50.60 \\
SH  & 0.109 & 0.57 & 0.023 & 0.43 & 2.395 & 0.00 & 0.594 & 0.00 & 0.016 & 0.00 & 0.012 & 0.00 & 0.039 &  0.13 \\ 
S   & 0.205 & 0.57 & 0.039 & 0.43 & 1.205 & 0.00 & 7.919 & 0.00 & 0.010 & 0.00 & 0.011 & 0.00 & 0.043 &  0.00 \\
\end{tabular}}
    \caption{ATE RMSE [m] and missing time [s] of the tested sequences \textbf{without added noise}. Each experiment is 60 seconds long.}
    \label{tab:slamgt}
\end{table*}


\subsection{Released Data}
\label{subsec:reldata}
We release 344 main sequences of 1800 frames each which, at 30 fps, correspond to 344 minutes of videos. In addition to that, we release the ones from the other scenarios, i.e. additional 20K frames. Except for the savanna, which has animated zebras, and the iRotate experiment, which has been tested in a static environment, all the others include dynamic humans. For each sequence, we save high-resolution depth, RGB, and instance segmentation. Furthermore, we generate 2D tight and loose bounding boxes\footnote{\url{https://bit.ly/3ClB0fQ}}, 3D bounding boxes, and the corresponding camera poses. This information is saved with \textit{numpy} arrays. The \textit{rosbags} contains IMU readings, TF tree, joint states, low-resolution RGBD images, and robot's state. For each experiment, we provide the initial configuration of each asset, as well as the state of the random number generator used, the USD file of the simulation, and other accompanying information necessary to replay the experiment. Other data such as normals, optical flow, SMPL vertices location and skeleton joint positions can be automatically generated given the provided data. All the USD files of the animated sequences (CLOTH3D) and environments, can be freely downloaded upon acceptance of the necessary licenses, or generated from scratch where necessary (AMASS). The source code necessary to i) convert environments and ii) the animated sequences, iii) manage the simulation (including the assets placement), iv) control the robots, v) post-process the data, vi) process the USD files to correct absolute paths, vii) replay the experiments and viii) SLAM libraries installation and testing, are provided as open source. Finally, we release the checkpoints of the trained networks alongside the data used to train them, the \textit{rosbags} used for the evaluation of the SLAM methods, and the TUM labelled sequences.

==> known_issues.tex <==
\section{LIMITATIONS AND FUTURE WORKS}
\label{sec:issues}
\textbf{Semantic segmentation}
Semantic segmentation of Front3D assets is notoriously faulty in some instances\footnote{\url{https://bit.ly/3ClC7w2}}. We modified the \textit{blenderproc} loader to have better mappings by assigning additional labels to each object. Still, we recognize that this is not sufficient. However, humans and flying objects are always labelled correctly.

\textbf{Realism and diversity} GRADE is designed to be modular and easily configurable. Visual realism is something that can be improved. This includes both the quality of the assets/textures (for environments and humans) and the variability of body shapes and movements. Moreover, rooms show only occidental-like designs which are always clean, squared, and uncluttered. Placement should also be improved with more advanced strategies, e.g. by considering semantic information to avoid humans sitting on plain air. Furthermore, variability  in the camera sensor settings and more diverse camera's movements should be used. Considering the code modularity, it would not be hard to include human or robot environment interactions or introduce animated pets (e.g. dogs, cats) and multi-level houses. The inclusion of motion generation software such as~\cite{samp} is also a direction that could be considered.

\textbf{Known Isaac Sim issues} We encountered various issues using Isaac Sim. The three main ones are: i) the ROS clock is sometimes not published at the right instant\footnote{\url{https://bit.ly/3Qa3SNL}}, ii) dynamic meshes not fully supported\footnote{\url{https://bit.ly/3Ql3sEb} \url{https://bit.ly/3jOnBGB}}, iii) rendering not done in one step, iv) the 2D occupancy map might be partially incorrect. The first one is easily solved either by a post-processing step or by waiting for the topic to be published. The second one causes issues with 3D bounding boxes, which can be corrected offline using our code, and with animations' collision elements that are not created correctly. Finally, since Isaac Sim use a raycasting technique to generate the 2D map from a given point, sometimes it can happen that this results in partial 2D maps. This can be solved quickly by re-generating it if necessary.

\textbf{Movement speed} Due to an overlooked scaling factor, the physics of the drone is more comparable to a handheld camera device, with spikes in the acceleration components when movement changes. However, data is still physically plausible and usable. 
